Quantum Key Leasing for PKE and FHE with a Classical Lessor

In this work, we consider the problem of secure key leasing, also known as revocable cryptography (Agarwal et. al. Eurocrypt' 23, Ananth et. al. TCC' 23), as a strengthened security notion of its predecessor put forward in Ananth et. al. Eurocrypt' 21. This problem aims to leverage unclonable nature of quantum information to allow a lessor to lease a quantum key with reusability for evaluating a classical functionality. Later, the lessor can request the lessee to provably delete the key and then the lessee will be completely deprived of the capability to evaluate. In this work, we construct a secure key leasing scheme to lease a decryption key of a (classical) public-key, homomorphic encryption scheme from standard lattice assumptions. We achieve strong form of security where: * The entire protocol uses only classical communication between a classical lessor (client) and a quantum lessee (server). * Assuming standard assumptions, our security definition ensures that every computationally bounded quantum adversary could not simultaneously provide a valid classical deletion certificate and yet distinguish ciphertexts. Our security relies on the hardness of learning with errors assumption. Our scheme is the first scheme to be based on a standard assumption and satisfying the two properties above.

==> outline.tex <==

%\paragraph{Outline of Proof}

Proof outline. 
Will comment out later.






\section{Proof Draft}
Overall we are trying to achieve a reduction from parallel repeated NTCF encryption to a parallel repetition of a weekly verifiable 1-of-2 puzzle $\hat{\mathcal{Z}}^n = (G^n,V_2^n)$, where $V_2(p,v,\alpha_0,\alpha_1) = V(p,v,o,0,\alpha_0)\cdot V(p,v,o,1,\alpha_1)$.\\
The puzzle $\hat{\mathcal{Z}}$ has completeness $\eta=1$ and hardness $h=1/2$ and subsequently $\hat{\mathcal{Z}}^n$ has completeness $\eta=1$ and hardness $h=1/2^n$.
Assume an adversary A that can break the encryption (guess b'=b). Then there exists an adversary A' that breaks the security of the parallel repetition of the weekly verifiable 1-of-2 puzzle.

\begin{itemize}
    \item A' gets $(pk_1,\dots,pk_n)$ from $\hat{\mathcal{Z}}^n$ and feeds them to A.
    \item A computes $(y_1,\dots,y_n)$ and sends them to A.
    \item A provides deletion certificates $d_1,\dots,d_n$ where $d_i = d_i',d(x_{i,0}\oplus x_{i,1})$ such that of, $Pr[Ver[d_1,\dots,d_n]=1]\ge\epsilon_1=1-negl(\lambda)$.
    \item A' sends $ct=Enc(\mu),\mu\in\{0,1\}$ to A.
    \item A returns back $\mu'$, where $Pr[\mu'=\mu]\ge 1/2 + \epsilon_2$, where $\epsilon_2$ is non-negligible, as well as the leftover quantum state $\rho$
    \item Using Extractor from below we extract pre-images with probability $Pr[Extr[ct, \rho]=(x_{1,b},\dots,x_{n,b})\ge \epsilon_2'$
\end{itemize}
As a result, $Pr[V_2^n((pk_1,\dots,pk_n),(td_1,\dots,td_n),\alpha_0,\alpha_1) = 1] = \epsilon_1 \cdot \epsilon_2' > 1/2^n$, which breaks the security of the puzzle.
\\\\
Notes: $V_2$ poorly defined for weakly verifiable. %Alternative: build NTCF with parallel repetition from 1-of-2 puzzle with parallel repetition?\\Is A' succeeding that or $\epsilon\cdot \epsilon_2 \ge 1/2+negl$?
\\ 
%First, the puzzle challenger runs $G^n(1^\lambda) \leftarrow \left ( (p_1,\dots,p_n), (v_1,\dots,v_n) \right ) $ and sends $(p_1,\dots,p_n)$ to A'. Then A' uses $(p_1,\dots,p_n)$ as the public keys and sends them to A, which in return calculates $y_1,\dots,y_n$ and $\rho_1,\dots,\rho_n$. 

%Afterwards, A deletes, providing $d_1,\cdots,d_n$. Then given ciphertext $ct_b = Enc(b)$ A' can guess b. Then using Theorem whatever, A' can use an extractor to get $x_b$.

%Finally A' retrieves both $(b,x_{b,1}),\dots, (b,x_{b,n})$ and $(c_1,d_1),\dots, (c_n,d_n)$
%$V^n ( (p_1,\dots,p_n), v_1,\dots,v_n, d_1,\dots,v_n, 0, (b,x_{b,1}),\dots, (b,x_{b,n})    ) = 1  $
%$V^n ( (p_1,\dots,p_n), v_1,\dots,v_n, d_1,\dots,v_n, 1, (c_1,d_1),\dots, (c_n,d_n)    ) = 1  $
%which breaks the puzzles security.
\subsection{Extraction} 

First we cosider the game where we ignore the certificate:
\begin{itemize}
    \item First, the challenger sends to the adversary the publik key $(A_1,A_1s_1+e_1,\dots,A_n,A_ns_n+e_n)$.
    \item The adversary computes and sends back $\{y_i=A_ix_i+e_i'\}_{i=1}^n$ as well as $\{d_i\}_{i=1}^n$. We call the residual state state $\rho_{del}$.
    \item The challenger checks that $y_i$ is well formed using the function $CHK_{FLWE}$. If $CHK_{FLWE}( (A_i,A_is_i+e_i),y_i,x_i) =1$, it continues, otherwise it outputs $\bot$.
    \item Then the challenger randomly picks between the following experiments:
    \begin{itemize}
        \item Exp 0: The challenger sends a ciphertext  $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{A_is_i+e_i\}_{i=1}^n \\ \sum y_i \end{bmatrix}\cdot R + \mu\cdot G$
        \item Exp 1: The challenger sends a matrix  $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{R_i\}_{i=1}^n \\ \sum_{i=1}^n y_i \end{bmatrix}$, where $R_i$ is random.
    \end{itemize}
\end{itemize}

We're going to show that experiment 0 and experiment 1 are computationally indistinguishable using a hybrid argument. 
\begin{itemize}
    \item Hybrid 0: The challenger sends $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{A_is_i+e_i\}_{i=1}^n \\ \sum_{i=1}^n y_i \end{bmatrix}\cdot R + \mu\cdot G$
    \item Hybrid 1: Instead of sending $A_1s_1+e_1$ the challenger sends a random value $R_1$. The two hybrids are indistinguishable due to the security of LWE. 
    \item Hybrid i:  Instead of sending $A_is_i+e_i$ the challenger sends a random value $R_i$. The two hybrids are indistinguishable due to the hardness of post-quantum LWE. 
    \item Hybrid N:  Instead of sending $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{A_is_i+e_i\}_{i=1}^n \\ \sum_{i=1}^n y_i \end{bmatrix}\cdot R + \mu\cdot G$ the challenger sends $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{R_i\}_{i=1}^n \\ \sum_{i=1}^n y_i \end{bmatrix}\cdot R + \mu\cdot G$. The two hybrids are indistinguishable due to the hardness of post-quantum LWE.  
    \item Hubrid N+1: The challenger sends $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{R_i\}_{i=1}^n \\ \sum_{i=1}^n y_i \end{bmatrix}$. The last two hybrids are indistiguishable due to the security of the GSW encryption scheme.
\end{itemize}

It's easy to show a reduction from decision LWE to distinguishing experiment 0 and experiment 1.  Assume an adversary $A$ than given $\rho_{del}$ can distinguish the above experiments. Then we can construct an adversary $A'$ that  distinguishes between  $(A_j, x_jA_j+e_j)$ and $(A_j,r_j)$. $A'$ samples n-1 LWE instances $(A_i,A_ix_i+e_i)$ as well as n random matrices $R_i,R_j$, $i\ne j$. Then they construct Experiment 0 and Experiment 1 and send them to $A$. $A$ sends back the decision to $A'$. 

We observe that in reality the two experiments are distinguishable for the adversary in our case because Pr[Decryption in Exoeriment 1] = 0 and $|$Pr[Decryption in Experiment 0] - Pr[Decryption in Game 1]$|$ = $|$Pr[Decryption in Game 0] $|$ $=\epsilon_2>$ negl.

Using the quantum search-to-decision LWE theorem below, we can extract a preimage with probability 1-negl.
\\\\
%$Ver_1->$ verify certificate\\
%$Ver_2->$ verify correct guess encryption
%$|Pr[Ver_2(D_1)=1] - Pr[Ver_1(D_0)=1]| \simeq |Pr[Ver_2(D_0)=1] - Pr[Ver_1(D_0)=1]| \le negl$ due to the security of the encryption

%We continue with extraction from experiment 1, where the first part of the ciphertext is
%$\begin{bmatrix}
%A_1 \\ \vdots  \\ A_n \\ R_1 \\ \vdots \\ R_n \\ \sum_{i=1}^n y_i
%\end{bmatrix} \cdot R$.
%Using the Leftover Hash Lemma the above statistically indistinguishable from 
%$\begin{bmatrix}
%A_1 \\ \vdots  \\ A_n \\ A_1R_1 \\ \vdots \\ A_nR_n \\ \sum_{i=1}^n y_i
%\end{bmatrix} \cdot R$. 
%\\\\
%We define the following games:
%Game 0: the above matrix.\\
%Game j: Last row = $\sum_{i\ne j}y_i+r_j$ where $y_i = x_iA_i+e_i$
%\\\\
%It's easy to show a reduction from decision LWE to distinguishing games 0 and j. Assume an adversary A than can distinguish the above games. Then we can construct an adversary A' that  distinguishes between 
%$(A_j, x_jA_j+e_j)$ and $(A_j,r_j)$.  A' samples n-1 LWE instances $(A_i,A_ix_i+e_i)$ as well as n random matrices $R_i,R_j$, $i\ne j$. Then they construct Game 0 and Game j and send them to A. A sends back the decision to A'.
%\\\\
%We observe that in reality Game 0 and Game j are distinguishable because Pr[Decryption in Game i] = 0 and $|$Pr[Decryption in Game 0] - Pr[Decryption in Game i]$|$ = $|$Pr[Decryption in Game 0] $|$ $=\epsilon_2>$ negl.
%\\\\
Now we consider the game where the certificate is verified:
\begin{itemize}
    \item First, the challenger sends to the adversary the publik key $(A_1,A_1s_1+e_1,\dots,A_n,A_ns_n+e_n)$.
    \item The adversary computes and sends back $\{y_i=A_ix_i+e_i'\}_{i=1}^n$ as well as the certificates $\{d_i\}_{i=1}^n$. We call the post-measurement state $\rho_{del}$.
    \item The challenger checks that $y_i$ is well formed using the function $CHK_{FLWE}$[BCMVV18], as well as if the certificates are valid. If $CHK_{FLWE}( (A_i,A_is_i+e_i),y_i,x_i) =1,\; \forall i$, it continues, otherwise it outputs $\bot$. In addition, if $Ver(td_A,d_i)=1,\;\forall i$ then it continues, otherwise it outputs $\bot$.
    \item Then the challenger randomly picks between the following experiments:
    \begin{itemize}
        \item Exp 0: The challenger sends a ciphertext  $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{A_is_i+e_i\}_{i=1}^n \\ \sum_{i=1}^n y_i \end{bmatrix}\cdot R + \mu\cdot G$
        \item Exp 1: The challenger sends a ciphertext  $\begin{bmatrix} \{A_i\}_{i=1}^n \\ \{R_i\}_{i=1}^n \\ \{y_i\}_{i=1}^n \end{bmatrix}$
    \end{itemize}
    
\end{itemize}
%We are going to show that ?
We project the leftover state $\rho_{del}$ to a $(1/2 + \epsilon)$-good distinguisher $\rho_{del}'$ (cite [CLLZ21]). By the definition of the measurement, $Pr[\rho_{del}' \mbox{ is a good distinguisher}]=|Pr[D(\rho_{del}',0)=1] - Pr[D(\rho_{del}',1)=1]|=1-negl(\lambda)$.

\begin{align*}
&|Pr[A(Exp\;0)=1] - Pr[Pr[A(Exp\;1)=1]|= \\
&=Pr[\prod_{i=1}^nVer(td_i,d_i)\wedge \rho_{del}' \mbox{ is a good distinguisher}] \\
&= Pr[\prod_{i=1}^nVer(td_i,d_i) | \rho_{del}' \mbox{ is a good distinguisher}] \cdot Pr[\rho_{del}'\mbox{ is a good distinguisher}]] \\
&\ge Pr[\prod_{i=1}^nVer(td_i,d_i) | \rho_{del}' \mbox{ is a good distinguisher}] - negl(\lambda) \\
&= \epsilon_2 - negl(\lambda) > negl(\lambda)
\end{align*}
Since $\rho_{del}'$ is a good distinguisher, according to the above technique we can use it to extract a preimage $x_b$ with probability $Pr[Ext(\rho_{del}')=x_b]>1-negl(\lambda)$.\\
As a result we have 
\begin{align*}
&Pr[Ext(\rho_{del}')=x_b \wedge \prod_{i=1}^nVer(td_i,d_i)=1 ]\\
&= Pr[Ext(\rho_{del}')=x_b | \prod_{i=1}^nVer(td_i,d_i)] \cdot Pr[\prod_{i=1}^nVer(td_i,d_i)=1] \\
&\ge Pr[\prod_{i=1}^nVer(td_i,d_i)=1] - negl(\lambda)\\
&= \epsilon_2 - negl(\lambda) > negl(\lambda)
\end{align*}
\subsection{Quantum Search-to-Decision LWE}

Theorem 7.1 [BBK22]: Assume there exists a classical non-adaptive black-box reduction from solving a non-interactive
assumption Q to solving a non-interactive assumption P with a verifiably-polynomial image. Then there exists a quantum reduction from solving Q to quantumly solving P. This reduction is durable if the original classical reduction has positive advantage. (modify to say that if the advantage of Q doesn't depend on P classically, then quantum Q solver has advantage independent from Q, then quantum Q solver has the same advantage as the classical).

%verifiably-polynomial image: any instance has at most polynomial many solutions and that this can be verified . 

%Formally: 
Verifiably-polynomial image: a non-interactive assumption P has verifiably-polynomial image if  $\exists$ verifier K such that for any instance $x$ the set $Y_x = \{ y: K(1^\lambda),x,y)=1 \}$ of K valid solutions is at most size $poly(\lambda)$, and for any valid instance $x=G(1^\lambda,r)$ and solution V such that $V(1^\lambda,r,y) = 1$, it holds that $y\in Y_x$

LWE decision assumption: solution space is $\{0,1\}$, trivially satisfies verifiably polynomial image. 
positive advantage: positive distance between threshold \& solving prob, decision problem has threshold 1/2 

As a result he quantum LWE search problem will have the same advantage as the classical one.
\\\\
%Alternatively :
%[STHY23] Reduction: 
%restrictions: q prime \& we can verify from LWE instances whether it is the correct answer for the LWE problem given some input s' (test a candidate solution).\\
%Specifically, given that $\chi$ is over $\{-k,\dots,k\}$ then we can construct algorithm V that with probability 1 - o(n):
%$V(x)=1$ if $x=s$, 0 otherwise [Lemma 2]

%Theorem: Let q be a prime and $\chi$ be a probability distribution over $\{-k,\dots,k\}, k\ll q/2$, If there's a quantum $\epsilon-$Distinguisher for the delusional $LW_{n,m,q,\chi}$ then there's a quantum algorithm that solves search $LWE_{n,m',q,\chi}$ with probability 1-o(n), where $m'=\tilde{O}(mq/\epsilon).$


==> parallel_puzzle.tex <==

\section{Parallel Repetition of the NTCF-based Protocol}


%To see the relationship of NTCFs and 1-of-2 puzzle, we show a simple correspondence between them. \luowen{:thinkingdoge:}
\begin{construction}
  \label{construct:ntcf21o2}
  Let $\mathcal F$ be an NTCF.
  An 1-of-2 puzzle can be constructed as follows.
\begin{itemize}
\item The $\keygen$ algorithm in 1-of-2 puzzle generates a public key $k$ and a secret key (trapdoor) $t_k$ for NTCF $f_k = \{f_{k,b}: \mathcal{X} \to \mathcal{D}_\mathcal{Y} \}_{k \in \mathcal{K}_\mathcal{F}, b \in \{0,1\}}$. Let $\pk = k$ and $\sk = (k, t_k)$.  

%The $\keygen$ algorithm in 1-of-2 puzzle is generates a public key $k$ and a secret key (trapdoor) $t_k$ for NTCF $f_k = \{f_{k,b}: \{0,1\}^n \to \{0,1\}^m \}_{b \in \{0,1\}}$. 

\item The $\obligate$ algorithm prepares the evaluation of $f'_k$ (instead of $f_k$) on the uniform superposition over all inputs, measures the image register to obtain $y$ and apply $\mathcal{J}$ on the input.
Let $\rho$ be the post-measurement state of the input register, where $\rho \approx \ket\psi\bra\psi$, and
$$\ket\psi = \frac{1}{\sqrt{2}}(\ket{0}\ket{\mathcal{J}(x_0)} +\ket{1}\ket{\mathcal{J}(x_1)})\ket{y}.$$%\luowen{$\rho$ is a mixed state, but is followed by a pure state in $\approx$}
This is because $f_{k}$ has the trapdoor injective pair property and efficient range superposition property of $f'$; $\mathcal{J}$ is an injective procedure. 

\item $\solve(\pk, y, \rho, 0)$ corresponds to measuring the two registers in state $\rho$ in computational basis and outputting $\ans = (b, \mathcal{J}(x_b)), b \in \{0,1\}, x_b \in \{x_0, x_1\}$.

$\ver(\sk,y,0,\ans)$ takes in secret key $\sk = (k, t_k)$, an obligation value $y$, the challenge bit $b = 0$ and $\ans$. In this case $\ans = (b, v)$. The verification algorithm first obtains $x' = \mathcal{J}^{-1}(v)$ and outputs $1$ if and only if $y \in \supp(f_{k,b}'(x))$. 

\item $\solve(\pk, y, \rho, 1)$ corresponds to   measuring state in Hadamard basis and outputting the measurement result $\ans = (b,d)$. %where $d \in \{0,1\}^n $ and $c = d\cdot (x_0\oplus x_1)$. 

$\ver(\sk,y,1,\ans)$ takes in secret key $\sk = (k, t_k)$, an obligation value $y$, the challenge bit $b = 1$ and $\ans$.
In this case, $\ans = (b, d)$. It outputs $1$ if and only if $d \ne 0$ and $d \cdot (\mathcal{J}(x_0) + \mathcal{J}(x_1)) = b$. 
\end{itemize}
\end{construction}

%\qipeng{this is our construction, because we need an XZ-solver. So I change the construction a little bit, by forcing the computation $\mathcal{J}$ in the $\ver$. }
Overall we are trying to achieve a reduction from parallel repeated NTCF encryption to a parallel repetition of a weekly verifiable 1-of-2 puzzle $\hat{\mathcal{Z}}^n = (G^n,V_2^n)$, where $V_2(p,v,\alpha_0,\alpha_1) = V(p,v,o,0,\alpha_0)\cdot V(p,v,o,1,\alpha_1)$.\\



\jiahui{add 1-of-2 puzzle and 2-of-2 securitydefinition and thm that NTCF implies  security of 2-of-2 puzzle}

%\begin{definition}[1-of-2 puzzle]
%A 1-of-2 puzzle consists of four efficient algorithms: the puzzle generator G, an obligation algorithm O, a 1-of-2 solver S, and a verification algorithm V . G is a classical algorithm, V is a classical deterministic algorithm, and O and S are quantum algorithms, which are defined as followed:
%\begin{itemize}
%    \item G outputs, on security parameter $\lambda$, a random puzzle p along with some verification information $v$: $(p, v) \leftarrow G(1^\lambda)$.
%    \item O receives a puzzle p outputs an obligation  classical string o called
%    \item V is a deterministic efficient classical algorithm that, on input of a puzzle p, verification key v, and answer a, outputs either zero or one: $V (p, v, a) \in {0, 1}$.
%\end{itemize}
%\end{definition}


\begin{definition}[Weakly Verifiable 1-of-2 puzzle]
A system for weakly verifiable puzzles consists of a pair of efficient classical algorithms $\Tilde{\mathcal{Z}}=\mathrm{(G,V)}$ such that
\begin{itemize}
    \item The puzzle generator G outputs, on security parameter $\lambda$, a random puzzle p along with some verification information $v$: $(p, v) \leftarrow G(1^\lambda)$.
    \item The puzzle verifier V is a deterministic efficient classical algorithm that, on input of a puzzle p, verification key v, and answer a, outputs either zero or one: $V (p, v, a) \in {0, 1}$.
\end{itemize}
A weakly verifiable puzzle $\Tilde{\mathcal{Z}}$ is $1-h$-hard if, for any QPT algorithm S, there exists a negligible function $negl(\lambda)$ such that:
$$\Pr[(V(p,v,a)=1)_{(p,v)\leftarrow G(1^\lambda), a \leftarrow S(p)}] \le h(\lambda) + negl$$

%We also say that a weakly berifiable puzzle $\Tilde{\mathcal{Z}}$ has completeness $\eta=1$ such that 
%$$\Pr[(p, v) \leftarrow G(1^\lambda),]$$
\end{definition}

\begin{definition}[Repetition of weakly verifiable puzzles]
Let $\Tilde{\mathcal{Z}}=\mathrm{(G,V)}$ be a weakly verifiable puzzle system, and let $n:\mathbb{N}\rightarrow \mathbb{N}$. We denote by $G^n$ the algorithm that, on security parameter $\lambda$, runs $G(1^\lambda)$ $n(\lambda)$ times and outputs all the $n$ puzzles with their respective
verification keys:
$$((p_1,\dots,p_n), (v_1,\dots,v_n) ) \leftarrow G(1^\lambda)$$
where $(p_i,v_i)\leftarrow G(1^\lambda)$. $V^n$ receives n outputs inputs and accepts if and only if all n runs of V accept:
$$V^N((p_1,\dots,p_n),(v_1,\dots,v_n),(a_1,\dots,a_n)  ) = \Pi_{i=1}^{n}V(p_i,v_i.a_i)$$
\end{definition}

\begin{remark}
Given a 1-of-2 puzzle $\mathcal{Z}=\mathrm{(G,O,S,V)}$, we can define the weakly verifiable puzzle $\Tilde{\mathcal{Z}}=\mathrm{(G,V_2)}$. The parallel repetition of 1-of-2 puzzles $\mathcal{Z}$ is $1-h^n$ hard if and only if the parallel repetition of weakly verifiable puzzles $\Tilde{\mathcal{Z}}$ is $1-h^n$ hard.
\end{remark}

%The puzzle $\hat{\mathcal{Z}}$ has %completeness $\eta=1$ and 
%hardness $h=1/2$ and subsequently $\hat{\mathcal{Z}}^n$ has %completeness $\eta=1$ and 
%hardness $h=1/2^n$.
\begin{theorem}
There exists a reduction from a parallel repeated NTCF encryption scheme to a parallel repetition of a weakly veriable 1-of-2 puzlle $\Tilde{\mathcal{Z}}^n$.
\end{theorem}






















%%%%%%%%%%%%%Orestis draft
\iffalse
\begin{proof}


Assume an adversary A that can break the encryption with advantage $\epsilon_1 = 1-negl,\epsilon_2>negl$, which means in the security Game, $\Pr[\mathrm{Del}^n(\pk,\td,\cert)_{i} > e_1$, $i\in\{1,\dots,n\}$, and $\Pr[\mu \samp \{0,1\},\mathcal{A}(ct)=\mu]  \ge \frac{1}{2}+ e_2$. Then there exists an adversary $A'$ that breaks the security of the parallel repetition of the weekly verifiable 1-of-2 puzzle.

\begin{itemize}
    \item $A'$ gets $(pk_1,\dots,pk_n)$ from $\hat{\mathcal{Z}}^n$ and feeds them to $A$.
    \item $A$ computes $(y_1,\dots,y_n)$ and sends them to $A'$.
    \item $A$ provides deletion certificates $d_1,\dots,d_n$ %where $d_i = d_i',d(x_{i,0}\oplus x_{i,1})$ 
    such that $Pr[Ver[d_1,\dots,d_n]=1]\ge\epsilon_1$.
    \item $A'$ sends $ct=Enc(\mu),\mu\in\{0,1\}$ to $A$.
    \item $A$ returns back $\mu'$, where $Pr[\mu'=\mu]\ge 1/2 + \epsilon_2$, where $\epsilon_2$ is non-negligible, as well as the leftover quantum state $\rho$
    \item Using the Search-to-Decision LWE Extractor we extract pre-images with probability $\Pr[\mathrm{Extr}[ct, \rho]=(x_{1,b},\dots,x_{n,b})]\ge \epsilon_2'$
\end{itemize}
As a result, $Pr[V_2^n((pk_1,\dots,pk_n),(td_1,\dots,td_n),\alpha_0,\alpha_1) = 1] = \epsilon_1 \cdot \epsilon_2' > 1/2^n$, which breaks the security of the puzzle.
\end{proof}
\fi

\iffalse
\begin{lemma}[Security]
Based on the security aof a weakly-verifiable puzzle, the scheme introduced above is semantically secure, as defined below.
\end{lemma}
\begin{proof}
Lalala
\end{proof}
\fi

==> single.tex <==
\section{Singe Repetition Case}
\subsection{Parameters}
\begin{itemize}
    \item $n=\Omega(\ell logq +\lambda)$
    \item $m=\Theta(n logq )$ \textcolor{blue}{(GenTrap requires $\Omega(nlogq)$, LHL -hybrid 2- requires $O(nlogq)$)}
    \item $B_P = \frac{q}{2C_T\sqrt{mnlogq}}$, $B_V=\frac{B_P}{2^\lambda}$ where $C_T$ is the universal constant from the GenTrap algorithm
\end{itemize}


\jiahui{Orestis's version of a single instance construction. Will comment out later}
\subsection{Scheme Construction}
\jiahui{since we will only be using the parallel repeated construction. I'll be editing only the parallel repeated secrtion}
\begin{itemize}
    \item $\InKeyGen$($1^\lambda$): On input the security parameter $1^\lambda$, the Keygen algorithm has classical interaction between two parties (Alice and Bob) and works as follows:
    \begin{itemize}
        \item Alice (classical) samples a uniformly random matrix
    $A \samp \mathbb{Z}_q^{n \times m}$ along with a trapdoor $\td$ using the procedure $\mathrm{GenTrap}
(1^n,1^m,q)$. In addition, Alice samples $s\samp \{0,1\}^n $ and $e \samp D_{Z_q^m,B_V}$ and it sends $(A, sA+e)$ to Bob (quantum).
    \item Bob prepares the state $\left( \rho_\sk =  \frac{1}{\sqrt{2}}(\ket{0,x_0}+\ket{1,x_1}),\; y\right)$ where $y=f_0(x_0)=f_1(x_1)=x_bA+e_0+b(sA+e),\;e_0 \samp D_{Z_q^m,B_P},\;x_b\samp  \mathbb{Z}_q^n$ (according to [BCMVV21]), and sends y back to Alice. Alice checks that y is in the support of $f_b(x_b)$ by calculating $\mathrm{CHK}_\mathcal{F}(A, sA+e,b,x_b,y)$, where $x_b\leftarrow \mathrm{INV}(\td,b,y)$
   
    \item Alice returns the public key $\pk = (A,sA+e,y)$ and the trapdoor $\td$.% and secret key $\sk=(-x_b \| -b \|  1),\;b \in \{0,1\}$.
    \orestis{to do: define INV, CHK and f somewhere}
    \end{itemize}
    \item \textbf{Enc$(\pk,\mu)$}: On input a public key $\pk = (A,sA+e,y)$ and a plaintext $\mu \in \{0,1\}$ the algorithm samples $R\samp\{0,1\}^{m\times m}$ and calculates a ciphertext $\ct= \begin{bmatrix} A \\ sA+e \\ y \end{bmatrix}\cdot R + \mu \cdot G_{n+2}$ where $G_{n+2}$ is the gadget matrix of dimensions $(n+2)\times m$.
     %\item \textbf{Dec$(\sk, ct)$}: On input a ciphertext $\td$ and a secret key $\sk=(-x_b \| -b \|  1),\;b\samp\{0,1\}$, the algorithm computes  $\sk\cdot \ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T)$. If the result is closer to 0, output 0. If it is closer  to $\frac{q}{2}$, output 1.
     \item \textbf{Dec$(\rho, ct)$}: On input the quantum state $\rho_\sk = \left( \frac{1}{\sqrt{2}}(\ket{0,x_0}+\ket{1,x_1})\right)$ and a ciphertext $\ct$, apply the unitary $U$ such that $$\ket{\rho} \ket{0}\rightarrow \ket{\rho} \left(\ket{(-x_0 \| 0 \|  1) \cdot \ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T))}+ \ket{(-x_1 \| -1 \|  1) \cdot \ct \cdot  G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T))}\right)$$ and measure the second register in the computational basis.
     \item \textbf{Del}($\rho_\sk$): On input the quantum state $\rho_\pk = \frac{1}{\sqrt{2}}(\ket{0,x_0}+\ket{1,x_1})$, perform a Hadamard measurement on the second qubit, yielding a string $d\in \{0,1\}^n$, with the state collapsing to $ \frac{1}{\sqrt{2}}(\ket{0}+(-1)^c\ket{1})$, where $c=d\cdot (x_0\oplus x_1)$. A Hadamard basis of the leftover state yields c. Return $(d,c)$.
     
     \item \textbf{VerDel}($\td, (d,c)$): On input a deletion certificate $(d, c)$, and the trapdoor $\td$ output 1 if $c=d \cdot(J(x_0)\oplus J(x_1)(mod2))$ and 0 otherwise, where $J(x)$ returns the binary represantation of $x$ and $x_b\leftarrow \mathrm{INV}(\td,b,y)$

\end{itemize}

\subsection{Security and Correctness Proof}
\begin{lemma}[Correctness]
The scheme introduced above satisfies correctness
\end{lemma}
\begin{proof}

Verifying Deletion Correctness derives directly from \orestis{cite paper}. We focus on Decryption correctness. 
For completness, we first prove that Alice can also correctly decrypt a ciphertext.
Fix a public key $(A,sA+e,y)$ where $y=x_bA+e_0+b(As+e)$,  a trapdoor for a $\td$ and an input ciphertext $\ct= \begin{bmatrix} A \\ sA+e \\ y \end{bmatrix}\cdot R + \mu \cdot G_{n+2}$. Alice computes $x_b\leftarrow \mathrm{INV}(\td,b,y)$ and creates a secret key $\sk=(-x_b \| -b \|  1),\;b\samp\{0,1\}$. Then $\sk\cdot \ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T)$ is computed as shown below. If the result is closer to 0, output 0. If it is closer  to $\frac{q}{2}$, output 1.
    
\begin{align*}
    &sk \cdot ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T) \\
    &= \left( (-x_b \| -b \|  1) \cdot \begin{bmatrix} A \\ sA+e \\ y \end{bmatrix}\cdot R + \mu \cdot G_{n+2} \right ) \cdot  G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T) \\
    &= \left ( \left ( -x_bA-b(sA+e)+x_bA+e_0+b(As+e) \right )\cdot R + (-x_b \| -b \|  1)\cdot \mu \cdot G_{n+2} \right ) \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T)\\
    &= e_0\cdot R \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T) + \mu \cdot (-x_b \| -b \|  1)\cdot (\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T \\
    &= e_0\cdot R \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T) + \mu \\
    &= \hat{e} + \mu \cdot  \lfloor \frac{q}{2} \rfloor
\end{align*} 
With chosen parameters the error term $ \hat{e}$ is small enough so as to distinguish between 0 and 1. \textcolor{blue}{does this need more details?}
\jiahui{Need a coherent, i.e. "in superposition" version of the decryption algo}
\\\\
We continue to prove Decryption Correctness for Bob. Again we fix a public key $(A,sA+e,y)$ where $y=x_bA+e_0+b(As+e)$,  a quantum state $\rho_\sk = \left( \frac{1}{\sqrt{2}}(\ket{0,x_0}+\ket{1,x_1})\right)$ and an input ciphertext $\ct= \begin{bmatrix} A \\ sA+e \\ y \end{bmatrix}\cdot R + \mu \cdot G_{n+2}$.

Recall that the decryption algorithm applies the unitary
$U$ such that $$\ket{\rho} \ket{0}\rightarrow \ket{\rho} \left(\ket{(-x_0 \| 0 \|  1) \cdot \ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T))}+ \ket{(-x_1 \| -1 \|  1) \cdot \ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T))}\right).$$
By measuring the second register, it collapses to 
\begin{align*}
    &(-x_b \| -b \|  1)\cdot \ct \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T)) &  b\leftarrow\{0,1\}\\
    &= e_0\cdot R \cdot G^{-1}((\mathbf{0} \| \lfloor \frac{q}{2} \rfloor)^T) + \mu \\
    &= \hat{e} + \mu \cdot  \lfloor \frac{q}{2} \rfloor
\end{align*} 
and yields the correct result as above, while the first registrr $\rho$ stays intact.

\end{proof}

\begin{lemma}[Security]
Based on the hardness assumption of LWE, the scheme introduced above is semantically secure, as defined below.
\end{lemma}
\begin{proof}
Assume an adversary $\mathcal{A}$ and the following security game (\textbf{Game 1}):
\begin{itemize}
    \item The Challenger $\mathcal{C}$ and adversary $\mathcal{A}$ create $(\pk,\sk,\td)\leftarrow \mathrm{KeyGen(1^\lambda)}$.
    \item $\mathcal{A}$ sends back a deletion certificate $(d,c)$. 
    \item If $\Del(d,c)=\mathsf{Valid}$, $\mathcal{C}$ sends to $\ct=\mathcal{A}$ $\Enc(\mu),\;\mu\samp \{0,1\}$. Otherwise it aborts.
    \item $\mathcal{A}$ outputs a plaintext guess $\mu'$.
\end{itemize}
We will prove that the probability $\mu=\mu'$ is close to half, or $Pr[\mu \samp \{0,1\},\mathcal{A}(ct)=\mu]\le \frac{1}{2}+\negl(n)$. \textcolor{blue}{Assume for now that deletion certificate correct with probability 1.}

Assume that $Pr[\mathcal{A}(ct)=\mu \;|\; \mu \samp \{0.1\}]> \frac{1}{2}+\negl(n)$. We build an adversary $\mathcal{A'}$ that breaks the adaptive hardcore bit property:  
$\mathcal{A'}(c,d|\Del(c,d)=1)\rightarrow\{x_b\}_{b\leftarrow\{0,1\}}$.
\jiahui{not breaking adaptive hardcore bit, but breaking the soundness of 1-of-2 puzzle}

We show the following Hybrid argument:
\begin{itemize}
    \item Hybrid 0: The above (real) interaction, where the Challenger sends $\ct= \begin{bmatrix} A \\ sA+e \\ y \end{bmatrix}\cdot R + \mu \cdot G_{n+2}$.
    
%    \item Hybrid 1: The public key $\pk=(A,sA+e,y)$ along with the quantum state $\rho$ is generated non-interactively by the Challenger and sent to the Adversary. This would require that the Challenger is quantum, which is not necessarily the case, only for the purposes of the proof. \textcolor{blue}{I don't think this works / is needed}
    
    \item Hybrid 2: The Challenger sends $ \begin{bmatrix} R' \\ sR'+e' \\ x_0R'+e_0R \end{bmatrix}+\mu\cdot G$ instead of the ciphertext, where $R' \samp \mathbb{Z}_q^{m\times m}$.
    
    \item Hybrid 3: The Challenger sends $ \begin{bmatrix} R' \\ r \\ x_0R'+e_0R \end{bmatrix}+\mu\cdot G$, where $r\samp \mathbb{Z}_q^{1\times m}$. 
    
  \item Hybrid 4: The Challenger sends $ \begin{bmatrix} R' \\ r \\ x_0R'+e'' \end{bmatrix}+\mu\cdot G$, where $e'' \samp D_{Z_q^m,\sqrt{m}B_P}$.

    %\item Hybrid 5: The Challenger sends $ \begin{bmatrix} AR \\ sAR+eR \\ r' \end{bmatrix}+\mu\cdot G$. This is computationally indistinguishable due to the leftover hash lemma and the hardness of LWE.
\end{itemize}
Below we argue indistinguishability for the above hybrid distributions:
\begin{itemize}
    \item Hybrid 0 $\approx_c$ Hybrid 2: Computationally indistinguishability follows from the leftover hash lemma, given that $m=\Theta(nlogq) $
    
    \item Hybrid 2 $\approx_c$ Hybrid 3: Computationally indistinguishability follows from the hardness of LWE. 
    
   \item Hybrid 3 $\approx$ Hybrid 4: To begin with, since $s$ is binary $e_0 \samp D_{Z_q^m,B_P}$, $\| e_0R \| \le m\sqrt{m}B_P$. Thus, given that both $e_0$ and $R$ where sampled randomly $x_0R'+e_0R =  x_0R'+e''$, $e'' \samp D_{Z_q^m,\sqrt{m}B_P}$. 
    
\end{itemize}

Since Hybrid 0 and Hybrid 4 are indistinguishable, we can use the interaction in Hybrid 4 for the security game ($\mathrm{Game_1}$).
Now imagine the game ($\mathrm{Game_2}$) where the Challenger sends $ \begin{bmatrix} R' \\ r \\ r' \end{bmatrix}+\mu\cdot G$, where $r'\samp \mathbb{Z}_q^{1\times m}$. 

We see that $\mathcal{A'}$ can distinguish between $\mathrm{Game_1}$ and $\mathrm{Game_2}$. 
Given a ciphertext $\td$ that is uniformly randomly chosen from one of the two Games, it can decrypt the one from Game 0 with probability $>\frac{1}{2}+\negl$, and the one from Game 1 with exactly $\frac{1}{2}$ by guessing. More specifically
$$ \left |\; |Pr[\mathcal{A'}(\mathrm{Game_1})=0] - Pr[\mathcal{A'}(\mathrm{Game_1})=1]|-|Pr[\mathcal{A'}(\mathrm{Game_2})=0] - Pr[\mathcal{A'}(\mathrm{Game_2})=1]|\; \right | > \negl $$
where
\begin{align*}
&\left |\; |Pr[\mathcal{A'}(\mathrm{Game_1})=0] - Pr[\mathcal{A'}(\mathrm{Game_1})=1]|-|Pr[\mathcal{A'}(\mathrm{Game_2})=0] - Pr[\mathcal{A'}(\mathrm{Game_2})=1]|\; \right | \\
&\le \left |\; Pr[\mathcal{A'}(\mathrm{Game_1})=0] - Pr[\mathcal{A'}(\mathrm{Game_1})=1]-Pr[\mathcal{A'}(\mathrm{Game_2})=0] + Pr[\mathcal{A'}(\mathrm{Game_2})=1]|\; \right | \\
&\le |Pr[\mathcal{A'}(\mathrm{Game_1})=0] - Pr[\mathcal{A'}(\mathrm{Game_2})=0]| + |Pr[\mathcal{A'}(\mathrm{Game_1})=1] - Pr[\mathcal{A'}(\mathrm{Game_2})=1]|\; \\
\end{align*} 
and thus 
$$|Pr[\mathcal{A'}(\mathrm{Game_1})=0] - Pr[\mathcal{A'}(\mathrm{Game_2})=0]| + |Pr[\mathcal{A'}(\mathrm{Game_1})=1] - Pr[\mathcal{A'}(\mathrm{Game_2})=1]|> negl$$
which means at least one of the two terms is greater than negligible and as a result, \textbf{the two Games are distinguishable from $\mathcal{A'}$.}

It's easy to now show a \textbf{reduction from decision LWE to distinguishing Game 1 and Game 2}.  Assume that $\mathcal{A'}$ can distinguish the above Games. Then we can construct an adversary $\mathcal{A''}$ that  distinguishes between  $(R', x_0R'+e'')$ and $(R',r')$, $r'\samp \mathbb{Z}_q^{1\times m}$.  On an input $(R',z)$, $\mathcal{A''}$ samples %an LWE instance $(xR'+e)$, $e \samp D_{Z_q^m,\sqrt{m}B_P}$ as well as 
the random vector $r\samp \mathbb{Z}_q^{1\times m}$ and a bit $\mu \samp \{0,1\}$. 
Then they attempt to construct Game 1 as seen in Hybrid 4 and Game 2, assuming $z = x_0R'+e$, and send them to $\mathcal{A'}$. If $\mathcal{A'}$ has advantage in distinguishing them, then $z = x_0A+e_0$. Else, z is uniformly random.

According to the Theorem below, we have a quantum Search-to-Decision LWE reduction, with which the Adversary can extract $x_b$ with probability $1-\negl(n)$. Hence, we break the adaptive hardcore bit property and we reach a contradiction.
\end{proof}


\jiahui{ Will comment out above later}


==> trash.tex <==
\subsection{Correctness}
\paragraph{Decryption Correctness}

The above scheme satisfies decryption correctness.

\begin{proof}
By applying the decryption procedure, we will have:
     \begin{align*}
        & (-\mathbf{sk}) \cdot \ct \cdot \bG^{-1}  (\mathbf{0}^{nk+k+1} \vert \lfloor\frac{q}{2}\rfloor) \\
         & = \left(-\sum_{i \in [k]}\frac{1}{\sqrt{2}}(\ket{\bx_{i,0}\bA_i} + \ket{\bx_{i,1} \bA_i +(\bs_i \bA_i + \be_i})+\sum_{i \in [k]} \by_{i} \right) \cdot \bR\bG^{-1}(\mathbf{0} \vert \lfloor\frac{q}{2}\rfloor) \\
         & +  \sum_{i \in [k]} \be_{i}'' + \bsk \cdot \mu \bG \bG^{-1}(\mathbf{0} \vert \lfloor\frac{q}{2}\rfloor)
         \\
         & = \frac{1}{\sqrt{2^k}} \sum_{\mathbf{b} \in (\{0,1\}^k}\ket{(\sum_{i \in [k]} \mathbf{b}_i \cdot \be_{i} +\be_{i}' )\cdot \bR\bG^{-1}(\mathbf{0} \vert \lfloor\frac{q}{2}\rfloor)} + \sum_{i \in [k]} \be_{i}'' + \lfloor\frac{q}{2}\rfloor \cdot \mu %\be_{0,i}^\top + 
     \end{align*} 
\end{proof}
  %\jiahui{check the final error size after subtracting sum y}
Since we have $\lVert \sum_i (\be_{i}' + \be_{i}) \rVert \leq k\cdot \sqrt{m} \cdot B_{P}, \lVert \sum_i \be_{i}''  \rVert \leq k\cdot \sqrt{m} \cdot B_{P'}$ and $\lVert \sum_{i \in [k]} (\mathbf{b}_i \cdot \be_{i}' +\be_{i} )\cdot \bR\bG^{-1}(\mathbf{0} \vert \lfloor\frac{q}{2}\rfloor) \rVert + \sum_i \be_{i}'' \leq \frac{q}{4}$ for all $\bb \in \{0,1\}^k $, we will obtain $\mu$ with all but negligible probability.

        %\bI_{nk+k+1})
   

\paragraph{Reusability}
Reusability of the decryption key follows from correctness and the gentle measurement lemma \cite{aaronson2018shadow}. 

\paragraph{Deletion Verification Correctness} 
The first two steps in $\VerDel$ will pass for any honestly prepared $\{\by_i\}_{i \in [k]}$ with $(1-\negl(\lambda))$ probability.

The $\delete$ procedure will operate on the state $\rho_\sk$ as follows. 
For each $\frac{1}{\sqrt{2}}(\ket{0,\bx_{i,0}}+\ket{1,\bx_{i,1}})$, $i \in [k]$, the $\delete$ procedure will turn the state into:
\begin{align*}
& \frac{1}{\sqrt{2}} \sum \ket{0, \cJ(\bx_{i,0})}+\ket{1,\cJ(\bx_{i,1})} \text{ after applying $\cJ(\cdot)$} \\
& \to \frac{1}{\sqrt{2^{n+2}}} \sum_{\bd_i,b,u} (-1)^{\bd \cdot \cJ(x_{i,b}) \oplus ub} \ket{u} \ket{\bd_i} \text{ after QFT} \\
& = \frac{1}{\sqrt{2^{n}}} \sum_{\bd_i \in \{0,1\}^{\lceil n\log q \rceil}} (-1)^{\bd_i \cdot \cJ(\bx_{i,0})} \ket{\bd_i\cdot (\cJ(\bx_{i,0}) \oplus \cJ(\bx_{i,1}))} \ket{\bd_i}
\end{align*}
A measurement in the computational basis will give us result ($c_i = \bd_i \cdot (\cJ(\bx_{i,0}) \oplus \cJ(\bx_{i,1})), \bd_i$), for any $i \in [k]$. Correctness of deletion verification thus follows.

\begin{remark}
Note that in our construction, using $\td$ one can also decrypt. It is easy to define a decryption procedure using $\td$ by the $\mathsf{INV(\td,b, \by)}$-procedure  in \Cref{sec:ntcf_from_lwe}. We omit the details here.     
\end{remark}

\begin{remark}
    The extension to encrypting multi-bit message follows naturally from a parallel repetition of the  encryption above.
\end{remark}

\jiahui{mention extending to multi-bit, trivial}
